Biologically Inspired Dynamic Thresholds for Spiking Neural Networks

The dynamic membrane potential threshold, as one of the essential properties of a biological neuron, is a spontaneous regulation mechanism that maintains neuronal homeostasis, i.e., the constant overall spiking firing rate of a neuron. As such, the neuron firing rate is regulated by a dynamic spiking threshold, which has been extensively studied in biology. Existing work in the machine learning community does not employ bioinspired spiking threshold schemes. This work aims at bridging this gap by introducing a novel bioinspired dynamic energy-temporal threshold (BDETT) scheme for spiking neural networks (SNNs). The proposed BDETT scheme mirrors two bioplausible observations: a dynamic threshold has 1) a positive correlation with the average membrane potential and 2) a negative correlation with the preceding rate of depolarization. We validate the effectiveness of the proposed BDETT on robot obstacle avoidance and continuous control tasks under both normal conditions and various degraded conditions, including noisy observations, weights, and dynamic environments. We find that the BDETT outperforms existing static and heuristic threshold approaches by significant margins in all tested conditions, and we confirm that the proposed bioinspired dynamic threshold scheme offers homeostasis to SNNs in complex real-world tasks.

==> sections/definitions.tex <==

% formatting stuff

\definecolor{Gray}{rgb}{0.5,0.5,0.5}
\definecolor{darkblue}{rgb}{0,0,0.7}
\definecolor{orange}{rgb}{1,.5,0} % something readable but different from todo
\definecolor{red}{rgb}{1,0,0} % something readable but different from todo

\newcommand{\heading}[1]{\noindent\textbf{#1}}
%\newcommand{\comment}[1]{{\textcolor{orange}{#1}}}
\newcommand{\note}[1]{{{\textcolor{orange}{#1}}}}
\newcommand{\todo}[1]{{\textcolor{darkblue}{TODO: #1}}}
\newcommand{\changed}[1]{{\textcolor{blue}{#1}}}
%\newcommand{\removed}[1]{{\textcolor{Gray}{\sout{#1}}}}
\newcommand{\revision}[1]{{{#1}}}
\newcommand{\place}[1]{ \begin{itemize}\item\textcolor{darkblue}{#1}\end{itemize}}
\newcommand{\de}{\mathrm{d}}

% some traditional defintions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

% arash added these two
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

% text abbrevs
% \newcommand{\eg}{{\it e.g.}}
% \newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}

\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{{\mbox{\bf C}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

% lin alg stuff
\newcommand{\Span}{\mbox{\textrm{span}}}
\newcommand{\Range}{\mbox{\textrm{range}}}
\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Nullspace}{\mbox{\textrm{nullspace}}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}
%XXX dumb question: do we not use \diag(...) to form diagonal or
%block diagonal matrices?

% probability stuff
\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\erf}{\mathop{\bf erf}}

% convexity & optimization stuff
\newcommand{\Co}{{\mathop {\bf Co}}}
\newcommand{\co}{{\mathop {\bf Co}}}
% \newcommand{\Var}{\mathop{\bf var{}}}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}
\newcommand{\QED}{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\epi}{\mathop{\bf epi}}
%\newcommand{\hypo}{\mathop{\bf hypo}}

\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\Card}{\mathop{\bf card}}

\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
% \newcommand{\bd}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}
\newcommand{\xopt}{x^{\rm opt}}

%the following ones seem way too specialized to be here...
%let's omve them to a new file called defs2.tex or something like that
\newcommand{\Xb}{{\mbox{\bf X}}}
\newcommand{\xst}{x^\star}
\newcommand{\varphist}{\varphi^\star}
\newcommand{\lambdast}{\lambda^\star}
\newcommand{\Zst}{Z^\star}
\newcommand{\fstar}{f^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\xc}{x^\star}
\newcommand{\lambdac}{\lambda^\star}
\newcommand{\lambdaopt}{\lambda^{\rm opt}}

% defs for cones & generalized inequalities
%\newcommand{\K}{\mathcal{K}}
\newcommand{\geqK}{\mathrel{\succeq_K}}
\newcommand{\gK}{\mathrel{\succ_K}}
\newcommand{\leqK}{\mathrel{\preceq_K}}
\newcommand{\lK}{\mathrel{\prec_K}}
\newcommand{\geqKst}{\mathrel{\succeq_{K^*}}}
\newcommand{\gKst}{\mathrel{\succ_{K^*}}}
\newcommand{\leqKst}{\mathrel{\preceq_{K^*}}}
\newcommand{\lKst}{\mathrel{\prec_{K^*}}}
\newcommand{\geqL}{\mathrel{\succeq_L}}
\newcommand{\gL}{\mathrel{\succ_L}}
\newcommand{\leqL}{\mathrel{\preceq_L}}
\newcommand{\lL}{\mathrel{\prec_L}}
\newcommand{\geqLst}{\mathrel{\succeq_{L^*}}}
\newcommand{\gLst}{\mathrel{\succ_{L^*}}}
\newcommand{\leqLst}{\mathrel{\preceq_{L^*}}}
\newcommand{\lLst}{\mathrel{\prec_{L^*}}}

% Theorem definitions.
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}

% alg description --- not much for now!
\newenvironment{algdesc}%
{\begin{quote}}{\end{quote}}

% figures
\def\figbox#1{\framebox[\hsize]{\hfil\parbox{0.9\hsize}{#1}}}

% captions a la sirev
\makeatletter
\long\def\@makecaption#1#2{
   \vskip 9pt
   \begin{small}
   \setbox\@tempboxa\hbox{{\bf #1:} #2}
   \ifdim \wd\@tempboxa > 5.5in
        \begin{center}
        \begin{minipage}[t]{5.5in}
        \addtolength{\baselineskip}{-0.95pt}
        {\bf #1:} #2 \par
        \addtolength{\baselineskip}{0.95pt}
        \end{minipage}
        \end{center}
   \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}
   \fi
   \end{small}\par
}
\makeatother

% some commands & environments for making lecture notes
\newcounter{oursection}
\newcommand{\oursection}[1]{
 \addtocounter{oursection}{1}
 \setcounter{equation}{0}
 \clearpage \begin{center} {\Huge\bfseries #1} \end{center}
 {\vspace*{0.15cm} \hrule height.3mm} \bigskip
 \addcontentsline{toc}{section}{#1}
}
\newcommand{\oursectionf}[1]{  % for use with foiltex
 \addtocounter{oursection}{1}
 \setcounter{equation}{0}
 \foilhead[-.5cm]{#1 \vspace*{0.8cm} \hrule height.3mm }
 \LogoOn
}
\newcommand{\oursectionfl}[1]{  % for use with foiltex landscape
 \addtocounter{oursection}{1}
 \setcounter{equation}{0}
 \foilhead[-1.0cm]{#1}
 \LogoOn
}

% Matrices and vectors
\newcommand{\Mat}[1]    {{\ensuremath{\mathbf{\uppercase{#1}}}}} %Matrix 
\newcommand{\Vect}[1]   {{\ensuremath{\mathbf{\lowercase{#1}}}}} %Vector
\newcommand{\Vari}[1]   {{\ensuremath{\mathbf{\lowercase{#1}}}}} %Vector
\newcommand{\Id}				{\mathbb{I}} %Identity matrix
\newcommand{\Diag}[1] 	{\operatorname{diag}\left({ #1 }\right)} %Diagonalized matrix
\newcommand{\Opt}[1] 	  {{#1}_{\text{opt}}} %Optimal point of an optimization
\newcommand{\CC}[1]			{{#1}^{*}} %Convex conjugate
\newcommand{\Op}[1]     {\Mat{#1}} %Operator
\newcommand{\mini}[1] {{\mbox{argmin}}_{#1} \: \: } %Minimize w.r.t.
\newcommand{\argmin}[1] {\underset{{#1}}{\mathop{\rm argmin}} \: \: } %Minimize w.r.t.
\newcommand{\argmax}[1] {\underset{{#1}}{\mathop{\rm argmax}} \: \: } %Maximize w.r.t.  
\newcommand{\minimize}{\mathop{\rm minimize} \: \:}
\newcommand{\minimizeu}[1]{\underset{{#1}}{\mathop{\rm minimize}} \: }
\newcommand{\grad}      {\nabla}
\newcommand{\kron}{\otimes} %Pointwise multiplication

\newcommand{\gradt}     {\grad_\z}
\newcommand{\gradx}     {\grad_\x}
\newcommand{\Drv}     	{\Mat{D}} %Derivative operator
\newcommand{\step}      {\text{\textbf{step}}}
\newcommand{\prox}[1]   {\mathbf{prox}_{#1}}
\newcommand{\ind}[1]    {\operatorname{ind}_{#1}}
\newcommand{\proj}[1]   {\Pi_{#1}}
\newcommand{\pointmult}{\odot} %Pointwise multiplication
\newcommand{\rr}   {\mathcal{R}}

% notation for method
\newcommand{\Basis}{\Mat{D}}         		% Matrix basis
\newcommand{\Corr}{\Mat{C}}             % measurement matrix
\newcommand{\conv}{\ast} %Convolution
\newcommand{\meas}{\Vect{b}}            % measurement vector
\newcommand{\Img}{I}                    % transient image
\newcommand{\img}{\Vect{i}}             % vectorized image
\newcommand{\vv}{\Vect{v}}
\newcommand{\p}{\Vect{p}}
\newcommand{\Splitvar}{T}                % dual var
\newcommand{\splitvar}{\Vect{t}}         % dual vectorized var
\newcommand{\Splitbasis}{J}                % dual basis
\newcommand{\splitbasis}{\Vect{j}}         % dual vectorized basis
\newcommand{\var}{\Vari{z}} 

%Fourier notation
%\newcommand{\F}[1] {\hat{#1}}
\newcommand{\FT}[1]			{\mathcal{F}\left( {#1} \right)} %Fourier transform
\newcommand{\IFT}[1]			{\mathcal{F}^{-1}\left( {#1} \right)} %Inverse Fourier transform

%Optimization
\newcommand{\func}{f}
\newcommand{\fMat}{\Mat{K}}

\newcommand{\avar}{\Vari{v}} 
\newcommand{\aspvar}{\Vari{z}} 

\newcommand{\mask}{\Mat{M}}

\newcommand{\Pen}      		{F} %Penalty function
\newcommand{\cardset}     {\mathcal{C}}
\newcommand{\Dat}      		{G} %Dataterm function
\newcommand{\Reg}      		{\Gamma} %Regularizer spatial

% factorization
\newcommand{\Trans}{\mathbf{\uppercase{T}}} % target
\newcommand{\Ph}{\mathbf{\uppercase{\Phi}}} % target

\newcommand{\Tvec}{\Vect{T}} % target
\newcommand{\Bvec}{\Vect{B}} % factor 2

\newcommand{\Wt}{\Mat{W}} % weight

\newcommand{\Perm}{\Mat{P}} % Permutation matrix
\newcommand{\C}{\Mat{C}} % Blur

\newcommand{\DiagFactor}[1]     {\Mat{O}_{ #1 }}  %Matrix operator

% notation for method
\newcommand{\Proj}{\Mat{P}}             % projection matrix

% vector
\newcommand{\Vector}[1]{\mathbf{#1}}
% matrix
\newcommand{\Matrix}[1]{\mathbf{#1}}
% tensor
\newcommand{\Tensor}[1]{\boldsymbol{\mathscr{#1}}}
% unfolded tensor
\newcommand{\TensorUF}[2]{\Matrix{#1}_{(#2)}}

% Kronecker product of n matrices
\newcommand{\MatrixKP}[1]{\Matrix{#1}_{\otimes}}
\newcommand{\MatrixKPN}[2]{\Matrix{#1}_{\otimes}^{#2}}

% Khatri Rao product of n matrices
\newcommand{\MatrixKRP}[1]{\Matrix{#1}_{\odot}}
\newcommand{\MatrixKRPN}[2]{\Matrix{#1}_{\odot}^{#2}}

% Hadamard product and division
\newcommand{\HP}{\circ}
\newcommand{\HD}{\oslash}

% left and right tightly spaced double [[ brackets
\newcommand{\leftDB}{\left[ \! \left[}
\newcommand{\rightDB}{\right] \! \right]}

% transpose symbol
\newcommand{\transpose}{T}

%Strut
\newcommand*\sstrut[1]{\vrule width0pt height0pt depth#1\relax}

%Inline equations
\newcommand{\inlineeqnum}{\refstepcounter{equation}~~\mbox{(\theequation)}}
\newcommand{\eqname}[1]{\tag*{#1~(\theequation)}\refstepcounter{equation}}

%Method specific
\newcommand{\lambdas}{\boldsymbol{\lambda}}
\newcommand{\alb}{\boldsymbol{\alpha}} 	%Reflectivity
\newcommand{\depth}{\boldsymbol{z}} 	%Reflectivity
\newcommand{\albi}{\alpha} 	%Reflectivity
\newcommand{\depthi}{z} 	%Reflectivity
\newcommand{\ambient}{s}
\newcommand{\jitter}{w}
\newcommand{\z}{\Vect{z}} 							%Depth
\newcommand{\x}{\Vect{x}}             	% vectorized unknowns
\newcommand{\y}{\Vect{y}}             	% vectorized slack vars
\newcommand{\Kvar}{\Mat{K}}
\newcommand{\lagrangemult}{\boldsymbol{\nu}}
\newcommand{\scaledlagrange}{\Vect{u}}
\newcommand{\eps}{\epsilon}
\newcommand{\vp}{\Vect{v}}










